Ranking Handball Teams from Statistical Strength Estimation

In this work, we present a methodology to estimate the strength of handball teams using a statistical method. We propose the use of the Conway-Maxwell-Poisson distribution to model the number of goals scored by a team as a flexible discrete distribution which can handle situations of non equi-dispersion. From its parameters, we derive a mathematical formula to determine the strength of a team. We propose a ranking based on the estimated strengths to compare teams across different championships. Applied to female handball club data from European competitions over the season 2022/2023, we show that our new ranking can have an echo in real sports events and the results.

==> figures/tex/HandFeatImport.tex <==
\pgfplotstableread[col sep = comma]{figures/data/HandFeatImport.csv}\tabledm
\def\xlistmacro{}
\def\xliststring{}
\pgfplotstableforeachcolumnelement{index}\of\tabledm\as\entry{%
\xifinlist{\entry}{\xlistmacro}{}{
        \listxadd{\xlistmacro}{\entry}
        \edef\xliststring{\xliststring\entry,}
    }
}
\begin{tikzpicture}
    %\begin{axis}[
    % xlabel={Label},
    %ylabel={Count},
    %symbolic x coords/.expand once={\xliststring},
    %xmajorgrids=true,
    %x tick label style={rotate=60,anchor=east}
        %]
        %\addplot [ybar] table [x=feature, y=importance, col sep=comma] {\tabledm};
        %\end{axis}
        \begin{axis}[
            x tick label style={font=\footnotesize, draw=none, anchor=north},
            y tick label style={font=\footnotesize, draw=none, anchor=east},
            label style={font=\footnotesize, draw=none},
            width=0.8\linewidth, % changed size a bit
            height=0.8\linewidth,
            xbar, % not xbar interval
            bar width=5pt,
            %xmin=0.02, % does it make more sense to start at zero?
            %xmax=0.15, % reduced this a bit
            xlabel = Importance,
            axis x line=bottom,
            axis y line=left,
            enlarge y limits=0.01, % no need to enlarge x limits
            symbolic y coords/.expand once={\xliststring},
            ytick = data,
        %    y tick label style={rotate=45, anchor=east}, % I wouldn't use this
            %xticklabel style={
            %  /pgf/number format/fixed % no scientific notation for the smallest values
            %}
         ]
            \addplot[BlueUnilu, fill=BlueUnilu] table [y=index, x=importance, col sep=comma] {figures/data/HandFeatImport.csv};
        \end{axis}
\end{tikzpicture}

==> figures/tex/force_plot.tex <==

\begin{tikzpicture}
    \begin{axis}[
        colorbar, colormap name=greenred,
        % colorbar style={
        %         ylabel style={anchor=west, text width=3cm, rotate=270},
        %     },
        scatter,
        scatter src=x,
        only marks,
        clip mode=individual,
        scatter/@pre marker code/.append code={
                \pgfkeys{/pgf/fpu=true,/pgf/fpu/output format=fixed}
                \pgfmathsetmacro\negheight{-\pgfplotspointmeta}         
                \fill [draw=black] 
                (axis direction cs:0,0.3) rectangle (axis direction cs:\negheight,-0.3);
                \pgfplotsset{mark=none}
            },
        % legend style={at={(0.5,-0.15)}, anchor=north,legend columns=-1},
        legend columns=-1,
    %   symbolic y coords={\xliststring},
        ytick={0,...,28},
        yticklabels={Defense strength (away),Away international,Back age (avg),Goalie age (avg),Away locals,Goalie age (std),Back age (std),Importance,Wing height (std),Pivot age (std),Travel (km),Game (Hour),Game (DoW),Wing age (std),Days to final,Pivot height (std),Wing height (avg),Back height (std),Pivot age (avg),Goalie height (std),Goalie height (avg),Back height (avg),Home locals,Pivot height (avg),Attack strength (away),Wing age (avg),Defense strength (home),Home international,Attack strength (home))},
        x tick label style={font=\footnotesize, draw=none, anchor=north},
        y tick label style={font=\footnotesize, draw=none, anchor=east},
        label style={font=\footnotesize, draw=none},
        % width=\linewidth, % changed size a bit
        height=0.65\linewidth,
        xbar, % not xbar interval
        bar width=5pt,
        % xmin=0.1, % does it make more sense to start at zero?
        % xmax=0.65, % reduced this a bit
        xlabel = Goals,
        % scatter/use mapped color={draw=black,fill=mapped color},
        axis x line=bottom,
        axis y line=left,
        enlarge y limits=0.01, % no need to enlarge x limits
        % symbolic y coords/.expand once={\xliststring},
        % ytick = data,
        xticklabels={26,27,28,29,30,31,32,33,34,35,36}
    %    y tick label style={rotate=45, anchor=east}, % I wouldn't use this
        %xticklabel style={
        %  /pgf/number format/fixed % no scientific notation for the smallest values
        %}
    ]
    \addplot table[x=shaphome,y expr=\coordindex, col sep=comma] {figures/data/ForcePlotMetz.csv};
    \draw[thick] (0,0) -- (0,27);
    \node[black!50] at (0.55,28) {\footnotesize Prediction: 32 goals};
    \end{axis}
  \end{tikzpicture}
